Understanding the dynamic impact of COVID-19 through competing risk modeling with bivariate varying coefficients

The coronavirus disease 2019 (COVID-19) pandemic has exerted a profound impact on patients with end-stage renal disease relying on kidney dialysis to sustain their lives. Motivated by a request by the U.S. Centers for Medicare & Medicaid Services, our analysis of their postdischarge hospital readmissions and deaths in 2020 revealed that the COVID-19 effect has varied significantly with postdischarge time and time since the onset of the pandemic. However, the complex dynamics of the COVID-19 effect trajectories cannot be characterized by existing varying coefficient models. To address this issue, we propose a bivariate varying coefficient model for competing risks within a cause-specific hazard framework, where tensor-product B-splines are used to estimate the surface of the COVID-19 effect. An efficient proximal Newton algorithm is developed to facilitate the fitting of the new model to the massive Medicare data for dialysis patients. Difference-based anisotropic penalization is introduced to mitigate model overfitting and the wiggliness of the estimated trajectories; various cross-validation methods are considered in the determination of optimal tuning parameters. Hypothesis testing procedures are designed to examine whether the COVID-19 effect varies significantly with postdischarge time and the time since pandemic onset, either jointly or separately. Simulation experiments are conducted to evaluate the estimation accuracy, type I error rate, statistical power, and model selection procedures. Applications to Medicare dialysis patients demonstrate the real-world performance of the proposed methods.

==> CRM with BVC/preamble.tex <==
\usepackage{bm}
\usepackage{amssymb,mathtools}
\usepackage{natbib}
\usepackage{caption}
\usepackage{subcaption}
%\setcitestyle{citesep={}, aysep={,},yysep={;}}
\bibliographystyle{biom}
\usepackage[hyphens]{url}
\Urlmuskip=0mu plus 1mu\relax
\usepackage[linesnumbered, ruled]{algorithm2e}
% Note: to use algorithm2e, the following line in biom.cls must be commented out
% \newtheorem{algorithm}{Algorithm}%[theorem]
% \newtheorem{procedure}{Procedure}%[section]
\setlength{\paperheight}{11in} % required so as to use hyperref below
\usepackage{hyperref}
\hypersetup{
colorlinks=true,
linkcolor=red,
filecolor=magenta,
citecolor=blue,
urlcolor=blue
}
\usepackage{cleveref}
\Crefname{assumption}{Assumption}{Assumptions}
\usepackage{setspace}
% \onehalfspacing
\usepackage{tikz}
\usepackage{calc} % for simple arithmetic
\tikzset{>=latex} % for LaTeX arrow head

%\usepackage{titlesec}

%\titlespacing\section{0pt}{12pt plus 4pt minus 2pt}{0pt plus 2pt minus 2pt}
% \titlespacing\subsection{0pt}{12pt plus 4pt minus 2pt}{0pt plus 2pt minus 2pt}
% \titlespacing\subsubsection{0pt}{12pt plus 4pt minus 2pt}{0pt plus 2pt minus 2pt}

% \newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
% \def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
% % \theoremstyle{definition}
% % \newtheorem{assum}{Assumption}

\usepackage{bbm}
\usepackage{textcomp} % \textminus

\usepackage{multirow,multicol,makecell,booktabs}
%\usepackage{caption}
%\captionsetup[table]{skip=2.5pt}

\def\R{\textsf{R}}
\DeclareMathOperator*{\maximize}{maximize}
\newcommand{\st}{\text{subject to}}

\def\balpha{\bm{\alpha}}
\def\bbeta{\bm{\beta}}
\def\bvarepsilon{\bm{\varepsilon}}
\def\bgamma{\bm{\gamma}}
\def\bdelta{\bm{\delta}}
\def\beeta{\bm{\eta}}
\def\btheta{\bm{\theta}}
\def\blambda{\bm{\lambda}}
\def\bmu{\bm{\mu}}
\def\brbmu{\Breve{\bm{\mu}}}
\def\bnu{\bm{\nu}}
\def\brho{\bm{\rho}}
\def\bPi{\bm{\Pi}}
\def\bLambda{\bm{\Lambda}}
\def\bSigma{\bm{\Sigma}}
\def\bGamma{\bm{\Gamma}}
\def\bOmega{\bm{\Omega}}
\def\bPsi{\bm{\Psi}}
\def\bPhi{\bm{\Phi}}

\def\Exp{\mathrm{E}}
\def\Var{\mathrm{Var}}
\def\Cov{\mathrm{Cov}}
\def\Corr{\mathrm{Corr}}
\def\GEE{\mathrm{GEE}}
\def\SRR{\mathrm{SRR}}
\def\CRF{\mathrm{CRF}}
\def\diag{\mathrm{diag}}
\def\vech{\mathrm{vech}}
\def\RS{\mathrm{RS}}
\def\MS{\mathrm{MS}}
\def\RW{\mathrm{RW}}
\def\MW{\mathrm{MW}}


\def\brmu{\Breve{\mu}}
\def\brd{\Breve{d}}
\def\brk{\Breve{k}}
\def\brt{\Breve{t}}
\def\bru{\Breve{u}}
\def\brx{\Breve{x}}
\def\brB{\Breve{B}}
\def\brC{\Breve{C}}
\def\brK{\Breve{K}}
\def\brT{\Breve{T}}
\def\brX{\Breve{X}}
\def\brbx{\Breve{\mathbf{x}}}
\def\brbB{\Breve{\mathbf{B}}}
\def\brbD{\Breve{\mathbf{D}}}
\def\brbI{\Breve{\mathbf{I}}}
\def\brbL{\Breve{\mathbf{L}}}
\def\brbX{\Breve{\mathbf{X}}}


\def\rd{\mathrm{d}}
\def\rB{\mathrm{B}}
\def\rF{\mathrm{F}}
\def\rM{\mathrm{M}}
\def\rP{\mathrm{P}}
\def\rR{\mathrm{R}}
\def\rS{\mathrm{S}}
\def\rW{\mathrm{W}}
\def\rD{\mathrm{D}}
\def\rC{\mathrm{C}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}
\def\bb{\mathbf{b}}
\def\bd{\mathbf{d}}
\def\bh{\mathbf{h}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\bt{\mathbf{t}}
\def\bx{\mathbf{x}}
\def\bv{\mathbf{v}}
\def\bz{\mathbf{z}}

\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cN{\mathcal{N}}
\def\cS{\mathcal{S}}
\def\cU{\mathcal{U}}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\hyp}{hyp}
\DeclareMathOperator{\prox}{\mathbf{prox}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\tr}{trace}
\def\vec{\mathrm{vec}}
\def\CVE{\mathrm{CVE}}
\def\diag{\mathrm{diag}}




